Continuous-Time Markov Decisions based on Partial Exploration

We provide a framework for speeding up algorithms for time-bounded reachability analysis of continuous-time Markov decision processes. The principle is to find a small, but almost equivalent subsystem of the original system and only analyse the subsystem. Candidates for the subsystem are identified through simulations and iteratively enlarged until runs are represented in the subsystem with high enough probability. The framework is thus dual to that of abstraction refinement. We instantiate the framework in several ways with several traditional algorithms and experimentally confirm orders-of-magnitude speed ups in many cases.

==> macros.tex <==
\usepackage{xparse}
\usepackage{mathtools}
\usepackage{environ}

% == LATEX
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

% == SPACE

%\usepackage{microtype}
%\renewcommand{\baselinestretch}{0.975} % >=0.97

%\newcommand{\spacefu}{\vspace*{-1.2em}}
%\newcommand{\spacefl}{\vspace*{-0.8em}}
%\newcommand{\myspace}{\vspace*{-0.5em}}

% == TODO

\NewDocumentCommand{\todo}{m}{%
	% Add to todo list
	\begin{tikzpicture}[remember picture, baseline=-0.75ex]%
	\node [coordinate] (inText) {};%
	\end{tikzpicture}%
	%
	% Make the margin par
	\marginpar{%
		\begin{tikzpicture}[remember picture, font=\scriptsize]%
		\draw node[draw=red, text width = 3.5cm, inner sep=0.3mm] (inNote){#1};%
		\end{tikzpicture}%
	}%
	\begin{tikzpicture}[remember picture, overlay]%
	\draw[draw=red]%
	([yshift=-0.2cm] inText)%
	% -| ([xshift=-0.05cm] inNote.west)%
	-| (inNote.south);%
	\end{tikzpicture}%
}%

% == SYMBOLS

\RequirePackage{marvosym}
\providecommand{\contradiction}{\Lightning}
\newcommand{\parm}{\mathord{\color{black!33}\bullet}}%


% == BOOLEAN

\newcommand{\boolor}{\vee}
\newcommand{\booland}{\wedge}
\newcommand{\boolOr}{\bigvee}
\newcommand{\boolAnd}{\bigwedge}
\newcommand{\boolnot}{\lnot}


% == BASIC OPERATORS

\DeclarePairedDelimiter{\delimabs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\delimnorm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\delimpospart}{\lgroup}{\rgroup^+}
\DeclarePairedDelimiter{\delimnegpart}{\lgroup}{\rgroup^-}
\DeclarePairedDelimiterX{\deliminner}[2]{\lange}{\rangle}{#1, #2}
\DeclarePairedDelimiter{\delimcardinality}{\lvert}{\rvert}
\DeclarePairedDelimiter{\delimset}{\lbrace}{\rbrace}
\DeclarePairedDelimiter{\delimtuple}{(}{)}
\DeclarePairedDelimiter{\delimlistt}{[}{]}
\DeclarePairedDelimiter{\delimfun}{(}{)}

\NewDocumentCommand{\abs}{sm}{\IfBooleanTF{#1}{\delimabs{#2}}{\delimabs*{#2}}}
\NewDocumentCommand{\norm}{sm}{\IfBooleanTF{#1}{\delimnorm{#2}}{\delimnorm*{#2}}}
\NewDocumentCommand{\pospart}{sm}{\IfBooleanTF{#1}{\delimpospart{#2}}{\delimpospart*{#2}}}
\NewDocumentCommand{\negpart}{sm}{\IfBooleanTF{#1}{\delimnetpart{#2}}{\delimnetpart*{#2}}}
\NewDocumentCommand{\inner}{sm}{\IfBooleanTF{#1}{\deliminner{#2}}{\deliminner*{#2}}}
\NewDocumentCommand{\cardinality}{sm}{\IfBooleanTF{#1}{\delimcardinality{#2}}{\delimcardinality*{#2}}}
\NewDocumentCommand{\set}{sm}{\IfBooleanTF{#1}{\delimset{#2}}{\delimset*{#2}}}
\NewDocumentCommand{\tuple}{sm}{\IfBooleanTF{#1}{\delimtuple{#2}}{\delimtuple*{#2}}}
\NewDocumentCommand{\closure}{sm}{\IfBooleanTF{#1}{\delimclosure{#2}}{\delimclosure*{#2}}}
\NewDocumentCommand{\listt}{sm}{\IfBooleanTF{#1}{\delimlistt{#2}}{\delimlistt*{#2}}}
\NewDocumentCommand{\fun}{smm}{\IfBooleanTF{#1}{{#2}\delimfun{#3}}{{#2}\delimfun*{#3}}}
\NewDocumentCommand{\funMacro}{smm}{\IfNoValueTF{#3}{#1}{\fun{#2}{#3}}}

\DeclareMathOperator{\ExistsOp}{\exists}
\DeclareMathOperator{\ForallOp}{\forall}

\NewDocumentCommand{\Exists}{gg}{\IfNoValueTF{#1}{\ExistsOp}{\ExistsOp #1. \, #2}}
\NewDocumentCommand{\Forall}{gg}{\IfNoValueTF{#1}{\ForallOp}{\ForallOp #1. \, #2}}


% == SETS OPERATORS

\newcommand{\setcomplement}[1]{{#1}^c}
\newcommand{\powerset}[1]{\mathcal{P}(#1)}

\newcommand{\unionSym}{\cup}
\newcommand{\unionBin}{\mathbin{\unionSym}}
\newcommand{\strictunionSym}{\dot{\unionSym}}
\newcommand{\strictunionBin}{\mathbin{\dot{\unionSym}}}
\newcommand{\intersectionSym}{\cap}
\newcommand{\intersectionBin}{\mathbin{\intersectionSym}}
\newcommand{\UnionSym}{\bigcup}
\newcommand{\UnionBin}{\mathbin{\UnionSym}}
\newcommand{\strictUnionSym}{\dot{\UnionSym}}
\newcommand{\strictUnionBin}{\mathbin{\strictUnionSym}}
\newcommand{\IntersectionSym}{\bigcap}
\newcommand{\IntersectionBin}{\mathbin{\IntersectionSym}}

\newcommand{\union}{\unionBin}
\newcommand{\strictunion}{\strictunionBin}
\newcommand{\intersection}{\intersectionBin}
\newcommand{\Union}{\UnionSym}
\newcommand{\strictUnion}{\strictUnionSym}
\newcommand{\Intersection}{\IntersectionSym}


% == BASIC SETS

\newcommand{\Continuous}{C}
\newcommand{\Sobolev}{\mathcal{W}}
\newcommand{\Naturals}{\mathbb{N}}
\newcommand{\Domain}{\mathfrak{D}}
\newcommand{\Measures}{\mathcal{M}}
\newcommand{\Lebesgue}{\mathcal{L}}
\newcommand{\Hilb}{H}
\newcommand{\Reals}{\mathbb{R}}
\newcommand{\Realsplus}{\mathbb{R}_{\geqslant 0}}
\newcommand{\Orlicz}{{\tilde{\Lebesgue}}}
\newcommand{\Distributions}{\mathcal{D}}


% == LIMITS

\NewDocumentCommand{\convto}{G{}}{\xrightarrow{#1}}
\NewDocumentCommand{\weakto}{G{}}{\xrightharpoonup{#1}}
\NewDocumentCommand{\weakstarto}{G{}}{\xrightharpoonup[*]{#1}}

% == OPERATORS

\newcommand{\gradient}{\nabla}
\newcommand{\laplacian}{\Delta}
\newcommand{\diff}{\partial}
\newcommand{\boundary}{\partial}
\DeclareMathOperator{\divergence}{div}
\DeclareMathOperator{\distance}{dist}
\DeclareMathOperator{\esssup}{ess sup}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\capacity}{cap}
\DeclareMathOperator{\signum}{signum}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\const}{const}
\DeclareMathOperator{\loc}{loc}
\DeclareMathOperator*{\argmax}{arg\, max}
\DeclareMathOperator{\opt}{opt}

\newcommand{\qee}{\hfill$\triangle$} % quod erat exemplandum % TODO del

% == LOGIC

\newcommand{\ltl}{\operatorname{LTL}}
\newcommand{\ctl}{\operatorname{CTL}}
\newcommand{\pctl}{\operatorname{pCTL}}
\newcommand{\Next}{\varbigcirc}
\newcommand{\until}{\, \mathcal{U}}
\newcommand{\wrel}{\mathcal{W}}
\newcommand{\lang}[1]{\mathcal{L}(#1)}
\newcommand{\reach}{\Diamond}
\newcommand{\treach}[1]{\reach^{\leqslant #1}}
\newcommand{\alws}{\Box}
\newcommand{\true}{\mathsf{true}}
\newcommand{\false}{\mathsf{false}}
\newcommand{\turn}{\mathsf{turn}}
\newcommand{\PQ}{\mathrm{PQ}}
\newcommand{\reachF}[3]{\probability_{\bowtie~#1}\left[ \reach^{\leqslant #2} #3 \right]} %#1 - probability threshold, #2 - timebound, #3 - goal set


% == COMPLEXITY
\newcommand{\NP}{\mathbf{NP}}
\newcommand{\NEXP}{\mathbf{NEXP}}
\newcommand{\PSPACE}{\mathbf{PSPACE}}

% == PROBABILITY
\NewDocumentCommand{\distributions}{d()}{\funMacro{\mathcal{D}}{#1}}
\newcommand{\probability}{\mathbb{P}}
\newcommand{\expectation}{\mathbb{E}}

% == MC, MPD, Games

\newcommand{\gain}{g} %value
\newcommand{\bias}{b}
\newcommand{\stat}{q}
\newcommand{\outcomes}{\mathcal{O}}
\newcommand{\salgebra}{\mathcal{F}}
\newcommand{\mevent}{\mathcal{E}}
\newcommand{\pmin}{p_{\min}}
\newcommand{\rmax}{r_{\max}}
\newcommand{\MECs}{\mathsf{MEC}}
\newcommand{\GCs}{\mathsf{GC}}

\newcommand{\Ts}{\mathcal{T}}
\newcommand{\Mc}{\mathsf{M}}
%\newcommand{\Mdp}{\mathcal{M}}
\newcommand{\Ctmdp}{\mathcal{M}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\Pm}{\mathbf{P}}

\newcommand{\ap}{Ap}
\newcommand{\states}{S}
\newcommand{\inv}{\nu}
\newcommand{\lab}{L}

\newcommand{\edges}{E}
\newcommand{\statesone}{S^N}
\newcommand{\statestwo}{S_2}
\newcommand{\statesp}{S^P}
\newcommand{\initstate}{s_\textrm{init}}
\newcommand{\initdist}{\mu}
\newcommand{\trans}{\Delta}
\newcommand{\av}{\mathsf{Av}}
\newcommand{\rew}{r}
\newcommand{\lu}{\hat{l},\hat{u}}

\newcommand{\exit}[1]{\lambda(#1)}
%\newcommand{\exitmax}[1]{\overline{\lambda}}
\newcommand{\exitmax}{\overline{\lambda}}
\newcommand{\ptime}[1]{\tau(#1)}

% = paths and strategies
\newcommand{\path}{\rho}
\newcommand{\paths}{\mathit{Paths}^*}
\newcommand{\pathsinf}{\mathit{Paths}}
\newcommand{\fpath}{w}
\newcommand{\Paths}{\Omega}
\newcommand{\straa}{\pi}
\newcommand{\straasim}{\pi_{\mathtt{sim}}}
\newcommand{\straauni}{\pi_\mathtt{uniform}}
\newcommand{\straaopt}{\overline{\pi}_\mathtt{opt}}
\newcommand{\lstraaopt}{\underline{\pi}_\mathtt{opt}}
\newcommand{\straas}{\Pi}
\newcommand{\plays}{\mathsf{Plays}}
\newcommand{\play}{\mathsf{Play}}
\newcommand{\last}[1]{#1\mathord\downarrow}
\newcommand{\first}[1]{#1\mathord\uparrow}

\newcommand{\GM}{\ensuremath{\mathit{Tim}}\xspace} %generalised measurable schedulers
\newcommand{\late}{\ell}	%late schedulers
\newcommand{\early}{e}		%early schedulers
\newcommand{\x}{\nabla}		%\x \in {\late, \early}


% = probability

\newcommand{\inits}{\hat s}
\NewDocumentCommand{\actions}{d()}{{\IfNoValueTF{#1}{\mathit{Act}}{\fun{\mathit{Act}}{#1}}}}
\newcommand{\pat}{\omega}
\newcommand{\Pat}{\mathsf{Runs}}
\newcommand{\fpat}{w}
\newcommand{\mem}{\mathsf{M}}
\newcommand{\Cone}{\mathsf{Cone}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\mec}{\mathsf{MEC}}
\newcommand{\scc}{\mathsf{SCC}}
\newcommand{\bscc}{\mathsf{BSCC}}

\newcommand{\attractor}{\mathsf{prob1}}
\newcommand{\pr}{\mathbb P}
\renewcommand{\Pr}[3]{\pr^{#1}\hspace{-0.16em}\left[{#3}\right]}   %\Pr{strat}{state}{event}
\newcommand{\PrS}[3]{\pr^{#1}_{#2}\hspace{-0.16em}\left[{#3}\right]}   %\Pr{strat}{state}{event}
\newcommand{\expected}{\mathbb{E}}
\newcommand{\expsucc}{\expected_\trans}
\newcommand{\Ex}[3]{\expected^{#1}_{#2}\hspace{-0.16em}\left[{#3}\right]}   %\Ex{strat}{state}{f}
\newcommand{\ExS}[3]{\expected^{#1}_{#2}\hspace{-0.16em}\left[{#3}\right]}   %\Ex{strat}{state}{f}


% == LOCAL

\newcommand{\push}{\mathrm{push}}
\newcommand{\pop}{\mathrm{pop}}
\newcommand{\topx}{\mathrm{top}}

 % == ALGORITHMS
\newcommand{\nSim}{\mathrm{n}_{\mathrm{sim}}}
\newcommand{\GetImportantPaths}[2]{\mathtt{GetImpPaths}(#1,#2)}
\newcommand{\SampleDiscretePath}[3]{\mathtt{SampleDiscretePath}(#1, #2, #3)}
\newcommand{\SamplePath}[3]{\mathtt{SamplePath}\ifblank{#3}{(#1, #2)}{(#1, #2, #3)}}
\newcommand{\ChooseScheduler}{\textsc{ChooseScheduler}}
\newcommand{\getRelevantSubset}[3]{\textsc{getRelevantSubset}\ifblank{#1}{\ifblank{#2}{\ifblank{#3}{}{(#1, #2, #3)}}{(#1, #2, #3)}}{(#1, #2, #3)}}
\newcommand{\evaluate}[2]{\mathtt{evaluate}(#1,#2)}

% == PROBLEM
%%\newcommand{\prr}[2]{\ifblank{#1}{\pr_{#2}}{\pr^{#1}_{#2}}}
%\newcommand{\reach}[2]{\Diamond^{\leq #1}#2}
\newcommand{\val}[3]{\textnormal{val}\ifblank{#2}{}{^{#2}}\ifblank{#1}{(#3)}{_{#1}(#3)}} %reachability value (ctmdp, state, T)
\newcommand{\der}[1]{\,\mathrm{d}#1}


\newcommand{\Algou}{\mathtt{Cool-Algo}}
\newcommand{\Algo}{\textsc{SubspaceTBR}}
\newcommand{\variance}{\sigma}
\newcommand{\disstep}{\delta}
\newcommand{\transdiscret}[1]{\Delta_{#1}}


% == CTMDP
\newcommand{\Act}{\mbox{Act}}
\newcommand{\Succ}{\mbox{Succ}}
\newcommand{\bfR}{{\bf R}}
\newcommand{\bfP}[2][]{\ifblank{#1}{\mathrm{Pr}_{#2}}{\mathrm{Pr}^{#1}_{#2}}}
\newcommand{\goals}{G}
\newcommand{\upperSub}[2]{\mathsf{upper}(#1, #2)}
\newcommand{\lowerSub}[2]{\mathsf{lower}(#1, #2)}

% == EXPERIMENTS
\newcommand{\tbn}{\texttt{D}}%{\texttt{TBN}}
\newcommand{\tbb}{\texttt{A}}%{\texttt{TBB}}
\newcommand{\tbu}{\texttt{U}}%{\texttt{TBU}}

\newcommand{\us}{{\mathsf{uni}}}
\newcommand{\itbn}{$\tbn_\us$}
\newcommand{\itbb}{$\tbb_\us$}
\newcommand{\itbu}{$\tbu_\us$}

\newcommand{\os}{\mathsf{opt}}
\newcommand{\itbnplus}{$\tbn_\os$}
\newcommand{\itbbplus}{$\tbb_\os$}
\newcommand{\itbuplus}{$\tbu_\os$}

\newcommand{\prism}{\texttt{PRISM}}
\newcommand{\imca}{\texttt{IMCA}}
\newcommand{\scoop}{\texttt{SCOOP}}

\newcommand{\ftwc}{\texttt{ftwc}}
\newcommand{\gfs}{\texttt{gfs}}
\newcommand{\erlang}{\texttt{erlang}}
\newcommand{\ps}{\texttt{ps}}
\newcommand{\sjs}{\texttt{sjs}}
\newcommand{\one}{\texttt{one}}
\newcommand{\all}{\texttt{all}}

